Effective and Efficient Conversation Retrieval for Dialogue State Tracking with Implicit Text Summaries

Few-shot dialogue state tracking (DST) with Large Language Models (LLM) relies on an effective and efficient conversation retriever to find similar in-context examples for prompt learning. Previous works use raw dialogue context as search keys and queries, and a retriever is fine-tuned with annotated dialogues to achieve superior performance. However, the approach is less suited for scaling to new domains or new annotation languages, where fine-tuning data is unavailable. To address this problem, we handle the task of conversation retrieval based on text summaries of the conversations. A LLM-based conversation summarizer is adopted for query and key generation, which enables effective maximum inner product search. To avoid the extra inference cost brought by LLM-based conversation summarization, we further distill a light-weight conversation encoder which produces query embeddings without decoding summaries for test conversations. We validate our retrieval approach on MultiWOZ datasets with GPT-Neo-2.7B and LLaMA-7B/30B. The experimental results show a significant improvement over relevant baselines in real few-shot DST settings.

==> tables/motivating_example.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.45\textwidth}{!}
    {\begin{tabular}{l}
    \toprule
         \textbf{User}: Text mom I will be back Cambridge today  \\
         \textbf{System}: Message sent.  \\
         \textbf{User}: What’s the weather there? \\
         \textbf{System}: Sunny \\
         \textbf{User}: Get me a train there this afternoon. \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.12in}
    \caption{A conversation between a user and system.}
    \vspace{-0.2in}
    \label{tab:motivating-example}
\end{table}
